Turbulent Gas in Lensed Planck-selected Starbursts at redshifts 1-3.5

Dusty star-forming galaxies at high redshift (1 < z < 3) represent the most intense star-forming regions in the Universe. Key aspects to these processes are the gas heating and cooling mechanisms. Although it is well known that these galaxies are gas-rich, little is known about the gas excitation conditions. Here we examine these processes in a sample of 24 strongly lensed star-forming galaxies identified by the \textit{Planck} satellite (LPs) at z ~ 1.1 - 3.5. We analyze 162 CO rotational transitions (ranging from Jupper = 1 - 12) and 37 atomic carbon fine-structure lines ([CI]) in order to characterize the physical conditions of the gas in sample of LPs. We simultaneously fit the CO and [CI] lines, and the dust continuum emission, using two different non-LTE, radiative transfer models. The first model represents a two component gas density, while the second assumes a turbulence driven log-normal gas density distribution. These LPs are among the most gas-rich, infrared (IR) luminous galaxies ever observed ($\mu_{\rm L}$L$_{\rm IR(8-1000\mu m) } \sim 10^{13-14.6} $\Lsun; $< \mu_{\rm L}$M$_{\rm ISM}> = 2.7 \pm 1.2 \times 10^{12}$ \Msun, with $\mu_{\rm L} \sim 10-30$ the average lens magnification factor). Our results suggest that the turbulent ISM present in the LPs can be well-characterized by a high turbulent velocity dispersion ($<\Delta V_{\rm turb}> \sim 100 $ \kms) and gas kinetic temperature to dust temperature ratios $<T_{\rm kin}$/$T_{\rm d}> \sim 2.5$, sustained on scales larger than a few kpc. We speculate that the average surface density of the molecular gas mass and IR luminosity $\Sigma_{\rm M_{\rm ISM}}$ $\sim 10^{3 - 4}$ \Msun pc$^{-2}$ and $\Sigma_{\rm L_{\rm IR}}$ $\sim 10^{11 - 12}$ \Lsun kpc$^{-2}$, arise from both stellar mechanical feedback and a steady momentum injection from the accretion of intergalactic gas.

==> 0-tab-Allweightedmeans-abridged.tex <==





%--------- ABRIDGED VERSIONS: 

% Please add the following required packages to your document preamble:
% \usepackage{graphicx}
\begin{table*}
%\centering
\resizebox{\textwidth}{!}{%
\begin{tabular}{|c|c|c|c|c|c|c|c|c|}
\hline
Parameter: &
  log($ n_{   H_{ \rm 2}  } $) &
  Err, log($ n_{   H_{ \rm 2}  } $) &
  $T_{\rm k}$ &
  Err, $T_{\rm k}$ &
  $R_{\rm eff}$ &
  Err, $R_{\rm eff}$ &
  $\Delta V_{\rm turb}$ &
  Err, $\Delta V_{\rm turb}$ \\ \hline
Source ID   & cm$^{-3}$ & cm$^{-3}$ & K        & K        & pc       & pc       & km / s   & km / s   \\ \hline
LPsJ0116-24 & 4.92E+00  & 3.82E+00  & 6.97E+01 & 3.29E+01 & 1.46E+04 & 2.48E+03 & 1.48E+02 & 3.56E+01 \\ \hline
LPsJ0209+00 & 5.86E+00  & 6.17E-01  & 4.34E+01 & 3.54E+00 & 1.61E+04 & 2.96E+03 & 3.58E+01 & 3.31E+01 \\ \hline
LPsJ0226+23 & 4.67E+00  & 4.83E+00  & 2.93E+02 & 7.32E+01 & 1.68E+04 & 3.13E+03 & 1.69E+02 & 3.42E+01 \\ \hline
LPsJ0305-30 & 4.76E+00  & 4.21E+00  & 1.18E+02 & 5.17E+01 & 9.33E+03 & 2.10E+03 & 1.68E+02 & 3.00E+01 \\ \hline
LPsJ0748+59 & 4.89E+00  & 3.79E+00  & 7.60E+01 & 2.46E+01 & 1.56E+04 & 2.42E+03 & 1.35E+02 & 3.58E+01 \\ \hline
LPsJ0846+15 & 4.01E+00  & 1.01E+01  & 1.06E+02 & 2.87E+01 & 1.42E+04 & 2.77E+03 & 1.45E+02 & 4.31E+01 \\ \hline
LPsJ1053+60 & 5.27E+00  & 7.90E-01  & 4.52E+01 & 3.68E+00 & 1.49E+04 & 2.76E+03 & 1.56E+02 & 3.85E+01 \\ \hline
LPsJ1053+05 & 4.05E+00  & 4.52E+00  & 1.37E+02 & 5.25E+01 & 1.45E+04 & 2.81E+03 & 9.83E+01 & 5.56E+01 \\  \hline
\end{tabular}%
}
\caption{Individual $\chi^{2}$ weighted mean and standard deviation values for the parameters derived in the Turbulence LVG models, based on evaluating $\sim $2 million model calculations. This table is published in its entirety in the machine-readable format. A portion is shown here for guidance regarding its form and content.  }
\label{tab:indmeansA}
\end{table*}







==> 01-dustphotometry-extended.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{longtable}
% Note: It may be necessary to compile the document several times to get a multi-page table to line up properly


\clearpage
\onecolumn



\begin{longtable}[c]{ccccc}
\hline
\multicolumn{1}{|c|}{Source:} &
  \multicolumn{1}{c|}{Frequency [GHz]} &
  \multicolumn{1}{c|}{Flux density [mJy]} &
  \multicolumn{1}{c|}{Error [mJy]} &
  \multicolumn{1}{c|}{Note} \\ \hline
\endfirsthead
\endhead
LPsJ0116   & 857  & 513  & 462  & Planck             \\
           & 545  & 555  & 336  & Planck             \\
           & 273  & 66   & 10   & ALMA/Band 6        \\
LPsJ0209   & 1199 & 880  & 27   & Herschel           \\
           & 856  & 991  & 30   & Herschel           \\
           & 600  & 773  & 33   & Herschel           \\
           & 353  & 167  & 25   & JCMT/SCUBA-2 850um \\
           & 278  & 154  & 6    & ACT                \\
           & 273  & 145  & 15   & LMT/AzTEC          \\
           & 218  & 69   & 3    & ACT                \\
           & 154  & 14   & 0.8  & ALMA/Band 4        \\
           & 148  & 17   & 2    & ACT                \\
           & 97   & 2    & 0.5  & ACT                \\
LPsJ0226   & 857  & 1804 & 1241 & Planck             \\
           & 545  & 1113 & 381  & Planck             \\
           & 353  & 433  & 185  & Planck             \\
           & 273  & 103  & 15   & LMT/AzTEC          \\
LPsJ0305   & 857  & 706  & 194  & Planck             \\
           & 545  & 375  & 177  & Planck             \\
           & 273  & 50   & 10   & LMT/AzTEC          \\
           & 272  & 48   & 7    & ALMA/Band 6        \\
LPsJ0748   & 857  & 997  & 593  & Planck             \\
           & 545  & 737  & 229  & Planck             \\
           & 353  & 351  & 133  & Planck             \\
           & 273  & 66   & 10   & LMT/AzTEC          \\
LPsJ0846   & 857  & 1748 & 322  & Planck             \\
           & 545  & 1167 & 240  & Planck             \\
           & 353  & 132  & 26   & JCMT/SCUBA-2       \\
           & 273  & 118  & 15   & LMT/AzTEC          \\
           & 272  & 76   & 11   & ALMA/Band 6        \\
LPsJ105322 & 1199 & 460  & 46   & Herschel           \\
           & 856  & 739  & 74   & Herschel           \\
           & 600  & 771  & 77   & Herschel           \\
           & 353  & 360  & 36   & JCMT/SCUBA-2       \\
           & 149  & 38   & 4    & IRAM/GISMO-2       \\
LPsJ105353 & 1199 & 1028 & 103  & Herschel           \\
           & 856  & 996  & 100  & Herschel           \\
           & 600  & 735  & 74   & Herschel           \\
           & 353  & 198  & 11   & JCMT/SCUBA-2       \\
           & 273  & 98   & 10   & LMT/AzTEC          \\
           & 149  & 19   & 2    & IRAM/GISMO-2       \\
           & 102  & 2    & 0.2  & ALMA/Band 3        \\
LPsJ112713 & 857  & 195  & 127  & Planck             \\
           & 545  & 150  & 125  & Planck             \\
LPsJ112714 & 1199 & 810  & 81   & Herschel           \\
           & 856  & 708  & 71   & Herschel           \\
           & 600  & 448  & 45   & Herschel           \\
           & 353  & 90   & 9    & JCMT/SCUBA-2       \\
           & 273  & 24   & 2    & LMT/AzTEC          \\
           & 149  & 8    & 1    & IRAM/GISMO-2       \\
LPsJ1138   & 857  & 232  & 145  & Planck             \\
           & 545  & 93   & 90   & Planck             \\
           & 353  & 57   & 50   & Planck             \\
           & 273  & 10   & 1.4  & ALMA/Band 6        \\
LPsJ1139   & 1199 & 300  & 30   & Herschel           \\
           & 856  & 397  & 40   & Herschel           \\
           & 600  & 341  & 34   & Herschel           \\
           & 353  & 111  & 12   & JCMT/SCUBA-2       \\
           & 273  & 58   & 12   & LMT/AzTEC          \\
           & 272  & 49   & 7    & ALMA/Band 6        \\
           & 149  & 9    & 1    & IRAM/GISMO-2       \\
LPsJ1202   & 1199 & 618  & 62   & Herschel           \\
           & 856  & 646  & 65   & Herschel           \\
           & 600  & 451  & 45   & Herschel           \\
           & 353  & 123  & 14   & JCMT/SCUBA-2       \\
           & 273  & 69   & 7    & LMT/AzTEC          \\
           & 149  & 7    & 1    & IRAM/GISMO-2       \\
LPsJ1322   & 857  & 717  & 191  & Planck             \\
           & 545  & 322  & 152  & Planck             \\
           & 272  & 13   & 2    & ALMA/Band 6        \\
LPsJ1323   & 1199 & 652  & 65   & Herschel           \\
           & 856  & 590  & 59   & Herschel           \\
           & 600  & 393  & 39   & Herschel           \\
           & 353  & 108  & 10   & JCMT/SCUBA-2       \\
           & 273  & 33   & 3    & LMT/AzTEC          \\
           & 149  & 4    & 1    & IRAM/GISMO-2       \\
LPsJ1326   & 1199 & 197  & 20   & Herschel           \\
           & 856  & 288  & 30   & Herschel           \\
           & 600  & 288  & 29   & Herschel           \\
           & 353  & 65   & 7    & SMA                \\
           & 273  & 28   & 4    & ALMA/Band 6        \\
LPsJ1329   & 857  & 1298 & 200  & Planck             \\
           & 667  & 604  & 86   & JCMT/SCUBA-2       \\
           & 545  & 692  & 100  & Planck             \\
           & 353  & 271  & 90   & Planck             \\
           & 353  & 127  & 11   & JCMT/SCUBA-2       \\
           & 273  & 60   & 10   & LMT/AzTEC          \\
           & 272  & 51   & 8    & ALMA/Band 6        \\
           & 115  & 2    & 0.3  & NOEMA              \\
LPsJ1336   & 857  & 670  & 140  & Planck             \\
           & 545  & 313  & 154  & Planck             \\
           & 353  & 166  & 82   & Planck             \\
           & 273  & 65   & 12   & LMT/AzTEC          \\
LPsJ1428   & 4283 & 34   & 6    & Spitzer/MIPS       \\
           & 1874 & 430  & 90   & Spitzer/MIPS       \\
           & 1199 & 315  & 32   & Herschel           \\
           & 856  & 239  & 24   & Herschel           \\
           & 856  & 226  & 45   & SHARC-II           \\
           & 600  & 135  & 14   & Herschel           \\
           & 353  & 22   & 1.5  & JCMT/SCUBA-1       \\
           & 273  & 14   & 2    & LMT/AzTEC          \\
LPsJ1449   & 857  & 668  & 166  & Planck             \\
           & 545  & 457  & 160  & Planck             \\
           & 353  & 230  & 107  & Planck             \\
           & 273  & 37   & 8    & LMT/AzTEC          \\
           & 272  & 37   & 7    & ALMA/Band 6        \\
LPsJ1544   & 1199 & 220  & 9    & Herschel           \\
           & 856  & 340  & 6    & Herschel           \\
           & 600  & 314  & 6    & Herschel           \\
           & 353  & 87   & 5    & JCMT/SCUBA-2       \\
           & 273  & 35   & 10   & LMT/AzTEC          \\
           & 149  & 7    & 2    & IRAM/GISMO-2       \\
LPsJ1607   & 1199 & 167  & 17   & Herschel           \\
           & 856  & 167  & 17   & Herschel           \\
           & 600  & 78   & 8    & Herschel           \\
           & 273  & 8    & 1    & LMT/AzTEC          \\
LPsJ1609   & 1199 & 568  & 57   & Herschel           \\
           & 856  & 693  & 69   & Herschel           \\
           & 600  & 512  & 51   & Herschel           \\
           & 353  & 191  & 16   & JCMT/SCUBA-2       \\
           & 273  & 74   & 7    & LMT/AzTEC          \\
           & 149  & 8    & 1    & IRAM/GISMO-2       \\
LPsJ2313   & 857  & 393  & 266  & Planck             \\
           & 545  & 234  & 224  & Planck             \\
           & 273  & 19   & 3    & LMT/AzTEC          \\
           & 272  & 26   & 4    & ALMA/Band 6       \\
\caption{Ancillary dust photometry for the LPs. This table is published in its entirety in the machine-readable format.
      A portion is shown here for guidance regarding its form and content.}\\
\label{tab:continuumdata}\\
\end{longtable}




\clearpage
\twocolumn






==> 01-summaryLPs-diffVersions.tex <==

\begin{table*}
\centering
\begin{tabular}{ccccccccc}
\hline
\multicolumn{1}{|c|}{ID} &
  \multicolumn{1}{c|}{RA} &
  \multicolumn{1}{c|}{DEC} &
  \multicolumn{1}{c|}{$z_{\rm fg}$} &
  \multicolumn{1}{c|}{$z_{<CO/[CI]>}$} &
  \multicolumn{1}{c|}{$\mu_{\rm L}$} &
  \multicolumn{1}{c|}{$\mu_{\rm L}^{\dagger}$} &
  \multicolumn{1}{c|}{Lens size} &
  \multicolumn{1}{c|}{Reference} \\ \hline
\multicolumn{1}{|c|}{} &
  \multicolumn{1}{c|}{J2000} &
  \multicolumn{1}{c|}{J2000} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{$ \prime \prime $} &
  \multicolumn{1}{c|}{} \\ \hline
LPsJ0116 &
  01:16:46.77 &
  -24:37:01.90 &
  0.4 &
  2.12453 &
  - &
  23 &
  $\sim$4.5$^{GG}$ &
  I \\
LPs-J0209 &
  02:09:41.3 &
  00:15:59.00 &
  0.202 &
  2.55274 &
  7 -- 22 &
  58 &
  $\sim$3$^{GG}$ &
  II, III, IV, V \\
\multicolumn{1}{l}{} &
  \multicolumn{1}{l}{} &
  \multicolumn{1}{l}{} &
  \multicolumn{1}{l}{} &
  \multicolumn{1}{l}{} &
  \multicolumn{1}{l}{} &
  \multicolumn{1}{l}{} &
  \multicolumn{1}{l}{} &
  VI, VII, VIII \\
LPs-J0226 &
  02:26:33.98 &
  23:45:28.3 &
  0.34 &
  3.11896 &
  - &
  40 &
  $\sim$3.5$^{GG}$ &
  I \\
LPs-J0305 &
  03:05:10.62 &
  -30:36:30.30 &
  0.1-0.5 &
  2.26239 &
  - &
  18 &
  $\sim$2$^{GG}$ &
  I \\
LPs-J0748 &
  07:48:51.72 &
  59:41:53.5 &
  0.402 &
  2.75440 &
  - &
  21 &
  $\sim$13$^{GC}$ &
  I, IX, X \\
LPs-J0846 &
  08:46:50.16 &
  15:05:47.30 &
  0.1 &
  2.66151 &
  - &
  27 &
  $\sim$10$^{GC}$ &
  I \\
LPs-J105322 &
  10:53:22.60 &
  60:51:47.00 &
  0.837 &
  3.54936 &
  5 -- 12 &
  41 &
  $\sim$6$^{GG}$ &
  I, XI, XII, XIII \\
LPs-J105353 &
  10:53:53.00 &
  05:56:21.00 &
  1.525 &
  3.00551 &
  9 -- 48 &
  20 &
  $\sim$1.5$^{GG}$ &
  II, XI, XIV, XV \\
\multicolumn{1}{l}{} &
  \multicolumn{1}{l}{} &
  \multicolumn{1}{l}{} &
  \multicolumn{1}{l}{} &
  \multicolumn{1}{l}{} &
  \multicolumn{1}{l}{} &
  \multicolumn{1}{l}{} &
  \multicolumn{1}{l}{} &
  XII, XIII, XVI \\
LPs-J112714 &
  11:27:14.50 &
  42:28:25.00 &
  0.33-0.35 &
  2.23639 &
  20 -- 35 &
  25 &
  $\sim$13$^{GC}$ &
  II, XI, XII \\
\multicolumn{1}{l}{} &
  \multicolumn{1}{l}{} &
  \multicolumn{1}{l}{} &
  \multicolumn{1}{l}{} &
  \multicolumn{1}{l}{} &
  \multicolumn{1}{l}{} &
  \multicolumn{1}{l}{} &
  \multicolumn{1}{l}{} &
  XIII, XVII \\
LPs-J112713 &
  11:27:13.44 &
  46:09:24.10 &
  0.415 &
  1.30365 &
  - &
  21 &
  $\sim$1.5$^{GG}$ &
  I \\
LPs-J1138 &
  11:38:05.53 &
  32:57:56.90 &
  0.6 &
  2.01833 &
  - &
  10 &
  $\sim$1$^{GG}$ &
  I \\
LPs-J1139 &
  11:39:21.74 &
  20:24:50.90 &
  0.57 &
  2.85837 &
  6 -- 8 &
  19 &
  $\sim$1$^{GG}$ &
  I, XI, XII \\
LPs-J1202 &
  12:02:07.60 &
  53:34:39.00 &
  0.212 &
  2.44160 &
  - &
  25 &
  $\sim$5-10$^{GC}$ &
  I, XI, XII \\
LPs-J1322 &
  13:22:17.52 &
  09:23:26.40 &
  - &
  2.06762 &
  - &
  20 &
  $\sim$10$^{GC}$ &
  I \\
LPs-J1323 &
  13:23:02.90 &
  55:36:01.00 &
  0.47 &
  2.41671 &
  9 -- 12 &
  25 &
  $\sim$10$^{GC}$ &
  II, XI, XII, XVI \\
LPs-J1326 &
  13:26:30.25 &
  33:44:07.40 &
  0.64 &
  2.95072 &
  4 -- 5 &
  33 &
  $\sim$1.5$^{GG}$ &
  I, XVIII, XIX \\
LPs-J1329 &
  13:29:34.18 &
  22:43:27.30 &
  0.443 &
  2.04008 &
  9 -- 13 &
  31 &
  $\sim$11$^{GC}$ &
  I, XX, XXI, XXII \\
LPs-J1336 &
  13:36:34.94 &
  49:13:13.60 &
  0.28 &
  3.25477 &
  - &
  24 &
  $\sim$1.5$^{GG}$ &
  I \\
LPs-J1428 &
  14:28:23.90 &
  35:26:20.00 &
  - &
  1.32567 &
  - &
  4 &
  $\sim$1$^{GG}$ &
  II, XXIII, XXIV \\
\multicolumn{1}{l}{} &
  \multicolumn{1}{l}{} &
  \multicolumn{1}{l}{} &
  \multicolumn{1}{l}{} &
  \multicolumn{1}{l}{} &
  \multicolumn{1}{l}{} &
  \multicolumn{1}{l}{} &
  \multicolumn{1}{l}{} &
  XXV, XXVI, XXVII \\
LPs-J1449 &
  14:49:58.59 &
  22:38:36.80 &
  - &
  2.15360 &
  - &
  8 &
  $\sim$10$^{GC}$ &
  I \\
LPs-J1544 &
  15:44:32.35 &
  50:23:43.70 &
  0.673 &
  2.59884 &
  10-17 &
  10 &
  $\sim$7$^{GC}$ &
  I, XI, XII \\
\multicolumn{1}{l}{} &
  \multicolumn{1}{l}{} &
  \multicolumn{1}{l}{} &
  \multicolumn{1}{l}{} &
  \multicolumn{1}{l}{} &
  \multicolumn{1}{l}{} &
  \multicolumn{1}{l}{} &
  \multicolumn{1}{l}{} &
  XIII, XXVIII \\
LPs-J1607 &
  16:07:22.6 &
  73:47:03 &
  0.65 &
  1.48390 &
  - &
  4 &
  $\sim$1$^{GG}$ &
  II \\
LPs-J1609 &
  16:09:17.80 &
  60:45:20.00 &
  0.45 &
  3.25550 &
  12 -- 16 &
  44 &
  $\sim$7$^{GC}$ &
  II, XI, XII \\
\multicolumn{1}{l}{} &
  \multicolumn{1}{l}{} &
  \multicolumn{1}{l}{} &
  \multicolumn{1}{l}{} &
  \multicolumn{1}{l}{} &
  \multicolumn{1}{l}{} &
  \multicolumn{1}{l}{} &
  \multicolumn{1}{l}{} &
  XIII, XVI \\
LPs-J2313 &
  23:13:56.64 &
  01:09:17.70 &
  0.56 &
  2.21661 &
  - &
  57 &
  $\sim$3$^{GG}$ &
  I \\ \hline
\end{tabular}%
\caption{Foreground lens redshfits as reported in references. $z_{<CO/[CI]>}$ is the average redshift of the \LPs\ based on all CO/[CI] line detections. $\mu_{\rm L}$ Lens magnfication factor range. Measured with single line / single-band CO / dust emission or HST near-IR imaging. $\mu_{\rm L}^{\dagger}$ = Estimated using ``Tully-Fisher'' method (see Appendix \ref{difflens}). $^{GG}$ = Galaxy-Galaxy lens. The lens arc size corresponds to the effective Einstein radius, or the inferred circular radius. $^{GC}$ = Galaxy-Galaxy Cluster (or group) lens. The lens arc size corresponds to the largest lens arclet or effective Einstein radius. \textbf{References:} I. Berman et al. (in prep), II. \citep{harrington2016}, III. \citep{harrington2019}, IV. \citep{geach2015}, V. \citep{su2017}, VI. \citep{geach2018}, VII. \citep{rivera2019}, VIII. Kamieneski et al. (in prep), IX. \citep{khatri2016}, X. \citep{amodeo2018}, XI. \citep{canameras2015}, XII. \citep{canameras2018b}, XIII. \citep{frye2019},  XIV. \citep{canameras2017a}, XV. \citep{canameras2017b}, XVI. \citep{harrington2018}, XVII. \citep{canameras2018a}, XVIII. \citep{bussmann2013}, XIX. \citep{yang2017}, XX. \citep{diaz-sanchez2017}, XXI. \citep{dannerbauer2019}, XXII. \citep{iglesias-groth2017}, XXIII. \citep{borys2006}, XXIV. \citep{iono2009}, XXV. \citep{sturm2010}, XXVI. \citep{stacey2010}, XXVII.  \citep{hailey-dunsheath2012}, XXVIII. \citep{nesvadba2019}}
\label{tab:summaryLPs}
\end{table*}









\begin{comment}

% Please add the following required packages to your document preamble:
% \usepackage{lscape}
% \usepackage{longtable}
% Note: It may be necessary to compile the document several times to get a multi-page table to line up properly
\begin{landscape}
\begin{longtable}[c]{cccccccc}
\hline
\multicolumn{1}{|c|}{ID} &
  \multicolumn{1}{c|}{RA} &
  \multicolumn{1}{c|}{DEC} &
  \multicolumn{1}{c|}{$z_{\rm fg}$} &
  \multicolumn{1}{c|}{$z_{<CO/[CI]>}$} &
  \multicolumn{1}{c|}{$\mu_{\rm L}$} &
  \multicolumn{1}{c|}{$\mu_{\rm L}^{\dagger}$} &
  \multicolumn{1}{c|}{Lens size} \\ \hline
\endhead
%
\multicolumn{1}{|c|}{} &
  \multicolumn{1}{c|}{J2000} &
  \multicolumn{1}{c|}{J2000} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{$ \prime \prime $} \\ \hline
LPsJ0116$^{I}$                                  & 01:16:46.77 & -24:37:01.90 & 0.4       & 2.12453 & -        & 23 & $\sim$4.5$^{GG}$  \\
LPs-J0209$^{II, III, IV, V, VI, VII, VIII}$     & 02:09:41.3  & 00:15:59.00  & 0.202     & 2.55274 & 7 -- 22  & 58 & $\sim$3$^{GG}$    \\
LPs-J0226$^{I}$                                 & 02:26:33.98 & 23:45:28.3   & 0.34      & 3.11896 & -        & 40 & $\sim$3.5$^{GG}$  \\
LPs-J0305$^{I}$                                 & 03:05:10.62 & -30:36:30.30 & 0.1-0.5   & 2.26239 & -        & 18 & $\sim$2$^{GG}$    \\
LPs-J0748$^{I, IX, X}$                          & 07:48:51.72 & 59:41:53.5   & 0.402     & 2.75440 & -        & 21 & $\sim$13$^{GC}$   \\
LPs-J0846$^{I}$                                 & 08:46:50.16 & 15:05:47.30  & 0.1       & 2.66151 & -        & 27 & $\sim$10$^{GC}$   \\
LPs-J105322$^{I, XI, XII, XIII}$                & 10:53:22.60 & 60:51:47.00  & 0.837     & 3.54936 & 5 -- 12  & 41 & $\sim$6$^{GG}$    \\
LPs-J105353$^{II, XI, XIV, XV, XII, XIII, XVI}$ & 10:53:53.00 & 05:56:21.00  & 1.525     & 3.00551 & 9 -- 48  & 20 & $\sim$1.5$^{GG}$  \\
LPs-J112714$^{II, XI, XII, XIII, XVII}$         & 11:27:14.50 & 42:28:25.00  & 0.33-0.35 & 2.23639 & 20 -- 35 & 25 & $\sim$13$^{GC}$   \\
LPs-J112713$^{I}$                               & 11:27:13.44 & 46:09:24.10  & 0.415     & 1.30365 & -        & 21 & $\sim$1.5$^{GG}$  \\
LPs-J1138$^{I}$                                 & 11:38:05.53 & 32:57:56.90  & 0.6       & 2.01833 & -        & 10 & $\sim$1$^{GG}$    \\
LPs-J1139$^{I, XI, XII}$                        & 11:39:21.74 & 20:24:50.90  & 0.57      & 2.85837 & 6 -- 8   & 19 & $\sim$1$^{GG}$    \\
LPs-J1202$^{I, XI, XII}$                        & 12:02:07.60 & 53:34:39.00  & 0.212     & 2.44160 & -        & 25 & $\sim$5-10$^{GC}$ \\
LPs-J1322$^{I}$                                 & 13:22:17.52 & 09:23:26.40  & -         & 2.06762 & -        & 20 & $\sim$10$^{GC}$   \\
LPs-J1323$^{II, XI, XII, XVI}$                  & 13:23:02.90 & 55:36:01.00  & 0.47      & 2.41671 & 9 -- 12  & 25 & $\sim$10$^{GC}$   \\
LPs-J1326$^{I, XVIII, XIX}$                     & 13:26:30.25 & 33:44:07.40  & 0.64      & 2.95072 & 4 -- 5   & 33 & $\sim$1.5$^{GG}$  \\
LPs-J1329$^{I, XX, XXI, XXII}$                  & 13:29:34.18 & 22:43:27.30  & 0.443     & 2.04008 & 9 -- 13  & 31 & $\sim$11$^{GC}$   \\
LPs-J1336$^{I}$                                 & 13:36:34.94 & 49:13:13.60  & 0.28      & 3.25477 & -        & 24 & $\sim$1.5$^{GG}$  \\
LPs-J1428$^{II, XXIII, XXIV, XXV, XXVI, XXVII}$ & 14:28:23.90 & 35:26:20.00  & -         & 1.32567 & -        & 4  & $\sim$1$^{GG}$    \\
LPs-J1449$^{I}$                                 & 14:49:58.59 & 22:38:36.80  & -         & 2.15360 & -        & 8  & $\sim$10$^{GC}$   \\
LPs-J1544$^{I, XI, XII, XIII, XXVIII}$          & 15:44:32.35 & 50:23:43.70  & 0.673     & 2.59884 & 10-17    & 10 & $\sim$7$^{GC}$    \\
LPs-J1607$^{II}$                                & 16:07:22.6  & 73:47:03     & 0.65      & 1.48390 & -        & 4  & $\sim$1$^{GG}$    \\
LPs-J1609$^{II, XI, XII, XIII, XVI}$            & 16:09:17.80 & 60:45:20.00  & 0.45      & 3.25550 & 12 -- 16 & 44 & $\sim$7$^{GC}$    \\
LPs-J2313$^{I}$                                 & 23:13:56.64 & 01:09:17.70  & 0.56      & 2.21661 & -        & 57 & $\sim$3$^{GG}$   \\ \hline
\centering
\caption{Foreground lens redshfits as reported in references. $z_{<CO/[CI]>}$ is the average redshift of LPs based on all CO/[CI] line detections. $\mu_{\rm L}^{\dagger}$ Lens magnfication factor range. Measured with single line / single-band CO / dust emission or HST near-IR imaging. $\dagger$ = Estimated using Tully-Fischer method -- Appendix \ref{difflens} $^{GG}$ = Galaxy-Galaxy lens. The lens arc size corresponds to the effective Einstein radius, or the inferred circular radius. $^{GC}$ = Galaxy-Galaxy Cluster (or group) lens. The lens arc size corresponds to the largest lens arclet or effective Einstein radius.
References: I. Berman et al. (in prep), II. \citep{harrington2016}, III. \citep{harrington2019}, IV. \citep{geach2015}, V. \citep{su2017}, VI. \citep{geach2018}, VII. \citep{rivera2019}, VIII. \citep{Kamieneski et al. (in prep)}, IX. \citep{khatri2016}, X. \citep{amodeo2018}, XI. \citep{canameras2015}, XII. \citep{canameras2018b}, XIII. \citep{frye2019},  XIV. \citep{canameras2017a}, XV. \citep{canameras2017b}, XVI. \citep{harrington2018}, XVII. \citep{canameras2018a}, XVIII. \citep{bussmann2013}, XIX. \citep{yang2017}, XX. \citep{diaz-sanchez2017}, XXI. \citep{dannerbauer2019}, XXII. \citep{iglesias-groth2017}, XXIII. \citep{borys2006}, XXIV. \citep{iono2009}, XXV. \citep{sturm2010}, XXVI. \citep{stacey2010}, XXVII.  \citep{hailey-dunsheath2012}, XXVIII. \citep{nesvadba2019}}
\label{tab:summaryLPs}\\
\end{longtable}
\end{landscape}


\end{comment}





\begin{comment}


% Please add the following required packages to your document preamble:
% \usepackage{lscape}
% \usepackage{longtable}
% Note: It may be necessary to compile the document several times to get a multi-page table to line up properly
\begin{landscape}
\begin{longtable}[c]{|l|c|c|c|c|c|c|c|c|}
\hline
ID &
  RA &
  DEC &
  $z_{\rm fg}$ &
  $z_{<CO/[CI]>}$ &
  $\mu_{\rm L}$ &
  $\mu_{\rm L}^{\dagger}$ &
  Lens size &
  Modelled Line / Continuum Data \\ \hline
\endhead
%
 &
  J2000 &
  J2000 &
   &
   &
   &
  $L'_{\rm CO(1-0)}$-FWHM Est. &
  $ \prime \prime $ &
   \\ \hline
LPsJ0116 &
  01:16:46.77 &
  -24:37:01.90 &
  0.4 &
  2.12453 &
  - &
  23 &
  $\sim$4.5$^{GG}$ &
  CO(J$_{\rm up}$ = 1,3,6,7,8,9,11$^{UL}$) \\ \hline
$^{I}$ &
   &
   &
   &
   &
   &
   &
   &
  [CI](J$_{\rm up}$ = 2) \\ \hline
 &
   &
   &
   &
   &
   &
   &
   &
  \textit{Planck} 857/545 GHz, ALMA 270 GHz \\ \hline
LPsJ0209 &
  02:09:41.3 &
  00:15:59.00 &
  0.202 &
  2.55274 &
  7 -- 22 &
  58 &
  $\sim$3$^{GG}$ &
  CO(J$_{\rm up}$ = 1,3,4,5,7,8,9,11) \\ \hline
$^{II, III, IV, V, VI, VII, VIII}$ &
   &
   &
   &
   &
   &
   &
   &
  [CI](J$_{\rm up}$ = 1,2) \\ \hline
 &
   &
   &
   &
   &
   &
   &
   &
  \textit{Herschel} 1200, 857, 600 GHz, JCMT 353 GHz \\ \hline
 &
   &
   &
   &
   &
   &
   &
   &
  ACT 278 GHz, LMT 273 GHz, ACT 218 GHz \\ \hline
 &
   &
   &
   &
   &
   &
   &
   &
  ALMA 155 GHz, ACT 148 GHz, CARMA 97 GHz \\ \hline
LPsJ0226 &
  02:26:33.98 &
  23:45:28.3 &
  0.34 &
  3.11896 &
  - &
  40 &
  $\sim$3.5$^{GG}$ &
  CO(J$_{\rm up}$ = 3,5,6,9,11,12) \\ \hline
$^{I}$ &
   &
   &
   &
   &
   &
   &
   &
  \textit{Planck} 857/545 GHz, LMT 273 GHz \\ \hline
LPsJ0305 &
  03:05:10.62 &
  -30:36:30.30 &
  0.1-0.5 &
  2.26239 &
  - &
  18 &
  $\sim$2$^{GG}$ &
  CO(J$_{\rm up}$ = 3,6,7,8,9) \\ \hline
$^{I}$ &
   &
   &
   &
   &
   &
   &
   &
  [CI](J$_{\rm up}$ = 2) \\ \hline
 &
   &
   &
   &
   &
   &
   &
   &
  \begin{tabular}[c]{@{}c@{}}\textit{Planck} 857/545 GHz, \\ \\ ALMA 270 GHz, LMT 273 GHz\end{tabular} \\ \hline
LPsJ0748 &
  07:48:51.72 &
  59:41:53.5 &
  0.402 &
  2.75440 &
  - &
  21 &
  $\sim$13$^{GC}$ &
  CO(J$_{\rm up}$ = 1,3,5,7,8,9) \\ \hline
$^{I, IX, X}$ &
   &
   &
   &
   &
   &
   &
   &
  [CI](J$_{\rm up}$ = 1,2) \\ \hline
 &
   &
   &
   &
   &
   &
   &
   &
  \textit{Planck} 857/545/353 GHz, LMT 273 GHz \\ \hline
LPsJ0846 &
  08:46:50.16 &
  15:05:47.30 &
  0.1 &
  2.66151 &
  - &
  27 &
  $\sim$10$^{GC}$ &
  CO(J$_{\rm up}$ = 1,3,4,5,7,8,11$^{UL}$) \\ \hline
$^{I}$ &
   &
   &
   &
   &
   &
   &
   &
  [CI](J$_{\rm up}$ = 1,2) \\ \hline
 &
   &
   &
   &
   &
   &
   &
   &
  \begin{tabular}[c]{@{}c@{}}\textit{Planck} 857/545/353 GHz, JCMT 353 GHz, \\ \\ ALMA 270 GHz, LMT 273 GHz\end{tabular} \\ \hline
LPsJ105322 &
  10:53:22.60 &
  60:51:47.00 &
  0.837 &
  3.54936 &
  5 -- 12 &
  41 &
  $\sim$6$^{GG}$ &
  CO(J$_{\rm up}$ = 3,4,5,6,7,9,10,11) \\ \hline
$^{I, XI, XII, XIII}$ &
   &
   &
   &
   &
   &
   &
   &
  [CI](J$_{\rm up}$ = 1,2) \\ \hline
 &
   &
   &
   &
   &
   &
   &
   &
  \textit{Herschel} 1200, 857, 600 GHz \\ \hline
 &
   &
   &
   &
   &
   &
   &
   &
  JCMT 353 GHz, IRAM30m 150 GHz \\ \hline
LPsJ105353 &
  10:53:53.00 &
  05:56:21.00 &
  1.525 &
  3.00551 &
  9 -- 48 &
  20 &
  $\sim$1.5$^{GG}$ &
  CO(J$_{\rm up}$ = 1, 3,4,5,6,7,8,9,10,11) \\ \hline
$^{II, XI, XIV, XV, XII, XIII, XVI}$ &
   &
   &
   &
   &
   &
   &
   &
  [CI](J$_{\rm up}$ = 1,2) \\ \hline
 &
   &
   &
   &
   &
   &
   &
   &
  \begin{tabular}[c]{@{}c@{}}\textit{Herschel} 1200, 857, 600 GHz, JCMT 353 GHz, \\ \\ LMT 273 GHz, IRAM30m 150 GHz, ALMA 100 GHz\end{tabular} \\ \hline
LPsJ112714 &
  11:27:14.50 &
  42:28:25.00 &
  0.33-0.35 &
  2.23639 &
  20 -- 35 &
  25 &
  $\sim$13$^{GC}$ &
  CO(J$_{\rm up}$ = 1, 3,4,6,7,8) \\ \hline
$^{II, XI, XII, XIII, XVII}$ &
   &
   &
   &
   &
   &
   &
   &
  [CI](J$_{\rm up}$ = 1,2) \\ \hline
 &
   &
   &
   &
   &
   &
   &
   &
  \begin{tabular}[c]{@{}c@{}}\textit{Herschel} 1200, 857, 600 GHz, JCMT 353 GHz, \\ \\  LMT 273 GHz, IRAM30m 150 GHz\end{tabular} \\ \hline
LPsJ112713 &
  11:27:13.44 &
  46:09:24.10 &
  0.415 &
  1.30365 &
  - &
  21 &
  $\sim$1.5$^{GG}$ &
  CO(J$_{\rm up}$ = 2, 3, 5) \\ \hline
$^{I}$ &
   &
   &
   &
   &
   &
   &
   &
  [CI](J$_{\rm up}$ = 1) \\ \hline
 &
   &
   &
   &
   &
   &
   &
   &
  \textit{Planck} 857/545 GHz \\ \hline
LPsJ1138 &
  11:38:05.53 &
  32:57:56.90 &
  0.6 &
  2.01833 &
  - &
  10 &
  $\sim$1$^{GG}$ &
  CO(J$_{\rm up}$ = 1, 2, 3,4,6,7, 9) \\ \hline
$^{I}$ &
   &
   &
   &
   &
   &
   &
   &
  [CI](J$_{\rm up}$ = 1,2) \\ \hline
 &
   &
   &
   &
   &
   &
   &
   &
  \textit{Planck} 857/545/353 GHz, ALMA 270 GHz \\ \hline
LPsJ1139 &
  11:39:21.74 &
  20:24:50.90 &
  0.57 &
  2.85837 &
  6 -- 8 &
  19 &
  $\sim$1$^{GG}$ &
  CO(J$_{\rm up}$ = 1, 3,5,7,8, 9, 10$^{UL}$) \\ \hline
$^{I, XI, XII}$ &
   &
   &
   &
   &
   &
   &
   &
  [CI](J$_{\rm up}$ = 1,2) \\ \hline
 &
   &
   &
   &
   &
   &
   &
   &
  \begin{tabular}[c]{@{}c@{}}\textit{Herschel} 1200, 857, 600 GHz, JCMT 353 GHz, \\ \\ LMT 273 GHz, ALMA 270 GHz, IRAM30m 150 GHz\end{tabular} \\ \hline
LPsJ1202 &
  12:02:07.60 &
  53:34:39.00 &
  0.212 &
  2.44160 &
  - &
  25 &
  $\sim$5-10$^{GC}$ &
  CO(J$_{\rm up}$ = 1, 3,4, 5,7,8, 9, 10) \\ \hline
$^{I, XI, XII}$ &
   &
   &
   &
   &
   &
   &
   &
  [CI](J$_{\rm up}$ = 1,2) \\ \hline
 &
   &
   &
   &
   &
   &
   &
   &
  \begin{tabular}[c]{@{}c@{}}\textit{Herschel} 1200, 857, 600 GHz, JCMT 353 GHz, \\ \\ LMT 273 GHz, IRAM30m 150 GHz\end{tabular} \\ \hline
LPsJ1322 &
  13:22:17.52 &
  09:23:26.40 &
  - &
  2.06762 &
  - &
  20 &
  $\sim$10$^{GC}$ &
  CO(J$_{\rm up}$ = 1, 2, 3,4,6,7, 8, 9) \\ \hline
$^{I}$ &
   &
   &
   &
   &
   &
   &
   &
  [CI](J$_{\rm up}$ = 1,2) \\ \hline
 &
   &
   &
   &
   &
   &
   &
   &
  \textit{Planck} 857/545 GHz, ALMA 270 GHz \\ \hline
LPsJ1323 &
  13:23:02.90 &
  55:36:01.00 &
  0.47 &
  2.41671 &
  9 -- 12 &
  25 &
  $\sim$10$^{GC}$ &
  CO(J$_{\rm up}$ = 1, 3,4,5, 6,7, 8, 10) \\ \hline
$^{II, XI, XII, XVI}$ &
   &
   &
   &
   &
   &
   &
   &
  [CI](J$_{\rm up}$ = 1,2) \\ \hline
 &
   &
   &
   &
   &
   &
   &
   &
  \begin{tabular}[c]{@{}c@{}}\textit{Herschel} 1200, 857, 600 GHz, JCMT 353 GHz, \\ \\ LMT 273 GHz, IRAM30m 150 GHz\end{tabular} \\ \hline
LPsJ1326 &
  13:26:30.25 &
  33:44:07.40 &
  0.64 &
  2.95072 &
  4 -- 5 &
  33 &
  $\sim$1.5$^{GG}$ &
  CO(J$_{\rm up}$ = 1, 3, 5, 6, 7, 8, 9, 12$^{UL}$) \\ \hline
$^{I, XVIII, XIX}$ &
   &
   &
   &
   &
   &
   &
   &
  [CI](J$_{\rm up}$ = 1,2) \\ \hline
 &
   &
   &
   &
   &
   &
   &
   &
  \begin{tabular}[c]{@{}c@{}}\textit{Herschel} 1200, 857, 600 GHz, \\ \\ SMA 353 GHz, ALMA 270 GHz\end{tabular} \\ \hline
LPsJ1329 &
  13:29:34.18 &
  22:43:27.30 &
  0.443 &
  2.04008 &
  9 -- 13 &
  31 &
  $\sim$11$^{GC}$ &
  CO(J$_{\rm up}$ = 1,2, 3, 4, 6, 7, 8, 9, 11) \\ \hline
$^{I, XX, XXI, XXII}$ &
   &
   &
   &
   &
   &
   &
   &
  [CI](J$_{\rm up}$ = 1,2) \\ \hline
 &
   &
   &
   &
   &
   &
   &
   &
  \begin{tabular}[c]{@{}c@{}}\textit{Planck} 857/545/353 GHz, JCMT 665/353 GHz, \\ \\ ALMA 270 GHz, LMT 273 GHz, NOEMA 115 GHz\end{tabular} \\ \hline
LPsJ1336 &
  13:36:34.94 &
  49:13:13.60 &
  0.28 &
  3.25477 &
  - &
  24 &
  $\sim$1.5$^{GG}$ &
  CO(J$_{\rm up}$ = 1, 3, 4, 5, 6, 8, 9, 10, 11) \\ \hline
$^{I}$ &
   &
   &
   &
   &
   &
   &
   &
  [CI](J$_{\rm up}$ = 1) \\ \hline
 &
   &
   &
   &
   &
   &
   &
   &
  \textit{Planck} 857/545/353 GHz, LMT 273 GHz \\ \hline
LPsJ1428 &
  14:28:23.90 &
  35:26:20.00 &
  - &
  1.32567 &
  - &
  4 &
  $\sim$1$^{GG}$ &
  CO(J$_{\rm up}$ = 1, 2, 3, 5) \\ \hline
$^{II, XXIII, XXIV, XXV, XXVI, XXVII}$ &
   &
   &
   &
   &
   &
   &
   &
  \begin{tabular}[c]{@{}c@{}}Spitzer 4283 / 1874 GHz, \textit{Herschel} 1200, 857, 600 GHz, \\ \\ Sharc-II 857 GHz, JCMT 353 GHz, LMT 273 GHz\end{tabular} \\ \hline
LPsJ1449 &
  14:49:58.59 &
  22:38:36.80 &
  - &
  2.15360 &
  - &
  8 &
  $\sim$10$^{GC}$ &
  CO(J$_{\rm up}$ = 1, 3, 4, 6, 7, 9) \\ \hline
$^{I}$ &
   &
   &
   &
   &
   &
   &
   &
  [CI](J$_{\rm up}$ = 1,2) \\ \hline
 &
   &
   &
   &
   &
   &
   &
   &
  \begin{tabular}[c]{@{}c@{}}\textit{Planck} 857/545/353 GHz, LMT 273 GHz, \\ \\ ALMA 270 GHz\end{tabular} \\ \hline
LPsJ1544 &
  15:44:32.35 &
  50:23:43.70 &
  0.673 &
  2.59884 &
  10-17 &
  10 &
  $\sim$7$^{GC}$ &
  CO(J$_{\rm up}$ = 1, 3, 4, 5, 7, 8) \\ \hline
$^{I, XI, XII, XIII, XXVIII}$ &
   &
   &
   &
   &
   &
   &
   &
  [CI](J$_{\rm up}$ = 1,2) \\ \hline
 &
   &
   &
   &
   &
   &
   &
   &
  \begin{tabular}[c]{@{}c@{}}\textit{Herschel} 1200, 857, 600 GHz, JCMT 353 GHz, \\ \\ LMT 273 GHz, IRAM30m 150 GHz\end{tabular} \\ \hline
LPsJ1607 &
  16:07:22.6 &
  73:47:03 &
  0.65 &
  1.48390 &
  - &
  4 &
  $\sim$1$^{GG}$ &
  CO(J$_{\rm up}$ = 1, 2, 3, 5) \\ \hline
$^{II}$ &
   &
   &
   &
   &
   &
   &
   &
  \begin{tabular}[c]{@{}c@{}}\textit{Herschel} 1200, 857, 600 GHz, \\ \\ LMT 273 GHz\end{tabular} \\ \hline
LPsJ1609 &
  16:09:17.80 &
  60:45:20.00 &
  0.45 &
  3.25550 &
  12 -- 16 &
  44 &
  $\sim$7$^{GC}$ &
  CO(J$_{\rm up}$ = 1, 3, 4, 5, 6, 8, 9, 10, 11) \\ \hline
$^{II, XI, XII, XIII, XVI}$ &
   &
   &
   &
   &
   &
   &
   &
  [CI](J$_{\rm up}$ = 1) \\ \hline
 &
   &
   &
   &
   &
   &
   &
   &
  \begin{tabular}[c]{@{}c@{}}\textit{Herschel} 1200, 857, 600 GHz, JCMT 353 GHz, \\ \\ LMT 273 GHz, IRAM30m 150 GHz\end{tabular} \\ \hline
LPsJ2313 &
  23:13:56.64 &
  01:09:17.70 &
  0.56 &
  2.21661 &
  - &
  57 &
  $\sim$3$^{GG}$ &
  CO(J$_{\rm up}$ = 1, 3, 4, 6, 7, 8, 11$^{UL}$) \\ \hline
$^{I}$ &
   &
   &
   &
   &
   &
   &
   &
  [CI](J$_{\rm up}$ = 1,2) \\ \hline
 &
   &
   &
   &
   &
   &
   &
   & \\ \hline
  \begin{tabular}[c]{@{}c@{}}\textit{Planck} 857/545 GHz, LMT 273 GHz, \\ \\ ALMA 270 GHz\end{tabular} \\ \hline
\caption{Foreground lens redshfits as reported in references. $z_{<CO/[CI]>}$ is the average redshift of LPs based on all CO/[CI] line detections.								
$\mu_{\rm L}^{\dagger}$ Lens magnfication factor range. Measured with single line / single-band CO / dust emission or HST near-IR imaging.								
$\dagger$ = Estimated using Tully-Fisher method, with an uncertainty of $\sim 30$\% -- Sec. \ref{adoptedunc} 						
$^{GG}$ = Galaxy-Galaxy lens. The lens arc size corresponds to the effective Einstein radius, or the inferred circular radius								
$^{GC}$ = Galaxy-Galaxy Cluster (or group) lens. The lens arc size corresponds to the largest lens arclet or effective Einstein radius.								
References: I. Berman et al. (in prep), II. \citep{harrington2016}, III. \citep{harrington2019}, IV. \citep{geach2015}, V. \citep{su2017}, VI. \citep{geach2018}, VII. \citep{rivera2019}, VIII. \citep{Kamieneski et al. (in prep)}, IX. \citep{khatri2016}, X. \citep{amodeo2018}, XI. \citep{canameras2015}, XII. \citep{canameras2018b}, XIII. \citep{frye2019},  XIV. \citep{canameras2017a}, XV. \citep{canameras2017b}, XVI. \citep{harrington2018}, XVII. \citep{canameras2018a}, XVIII. \citep{bussmann2013}, XIX. \citep{yang2017}, XX. \citep{diaz-sanchez2017}, XXI. \citep{dannerbauer2019}, XXII. \citep{iglesias-groth2017}, XXIII. \citep{borys2006}, XXIV. \citep{iono2009}, XXV. \citep{sturm2010}, XXVI. \citep{stacey2010}, XXVII.  \citep{hailey-dunsheath2012}, XXVIII. \citep{nesvadba2019}}
\label{tab:summaryLPs}\\
\end{longtable}
\end{landscape}






\end{comment}




==> AAStex/0-figs-spectra.tex <==
% Here we show all of the spectra available to our team. We refer the reader to \S \ref{theobs} for more details about the lines reported in the literature, which are used in our analyses, yet not shown here.\\

 

\begin{figure*}
\centering
 \includegraphics[scale = 0.25]{spectra/J0116-A-_allspec.png}
  \includegraphics[scale = 0.25]{spectra/J0116-B-_allspec.png}
 \includegraphics[scale = 0.23]{bestfit/J0116_line_dust_bestsolnsTURB.png}
  \includegraphics[scale = 0.23]{bestfit/J0116_line_dust_bestsolns2COMP.png}
  %\includegraphics[scale = 0.25]{hexbinTurb/TURBcomp1_hexbin_chisq_1_J0116.png}
 \caption{LPs-J0116}
 \label{fig:lines-0a}
\end{figure*}



\newpage
\begin{figure*}
\centering
 \includegraphics[scale = 0.38]{FIGS/J0116corner_plot.png}
  %\includegraphics[scale = 0.21]{hexbinTurb/TURBcomp1_hexbin_chisq_1_J0116.png}
 \caption{LPs-J0116. Posterior distributions of the explored solution space for the parameters used in the \textit{Turbulence} model. Denser regions indicate model calculations with higher likelihood. Note the parameters which are set free in the model, in contrast to those with tightened parameter limits. Contours represent the 16th and 84th percentiles in these likelihood distributions. The red points indicate the likelihood-weighted mean and standard deviation from $\sim$ 2 million model calculations.}
 \label{fig:lines-0b}
\end{figure*}
\newpage




\begin{figure*}
\centering
 \includegraphics[scale = 0.25]{spectra/J0209-A-_allspec.png}
 \includegraphics[scale = 0.25]{spectra/J0209-B-_allspec.png}
 \includegraphics[scale = 0.25]{spectra/J0209-C-_allspec.png}
 \caption{LPs-J0209}
 \label{fig:lines-1a}
\end{figure*}


\begin{figure*}
\centering
%  \includegraphics[scale = 0.25]{spectra/J0209-A-_allspec.png}
%  \includegraphics[scale = 0.25]{spectra/J0209-B-_allspec.png}
%  \includegraphics[scale = 0.25]{spectra/J0209-C-_allspec.png}
  \includegraphics[scale = 0.23]{bestfit/J0209_line_dust_bestsolnsTURB.png}
  \includegraphics[scale = 0.23]{bestfit/J0209_line_dust_bestsolns2COMP.png}
 \caption{LPs-J0209}
 \label{fig:lines-1b}
\end{figure*}
\newpage

\begin{figure*}
\centering
 \includegraphics[scale = 0.38]{FIGS/J0209corner_plot.png}
 \caption{LPs-J0209}
 \label{fig:lines-1c}
\end{figure*}
\newpage






\begin{figure*}
\centering
 \includegraphics[scale = 0.25]{spectra/J0226-A-_allspec.png}
 \includegraphics[scale = 0.25]{spectra/J0226-B-_allspec.png}
  \includegraphics[scale = 0.23]{bestfit/J0226_line_dust_bestsolnsTURB.png}
  \includegraphics[scale = 0.23]{bestfit/J0226_line_dust_bestsolns2COMP.png}
  %\includegraphics[scale = 0.25]{hexbinTurb/TURBcomp1_hexbin_chisq_1_J0226.png}
 \caption{LPs-J0226}
 \label{fig:lines-2a}
\end{figure*}


\newpage

\begin{figure*}
\centering
  \includegraphics[scale = 0.38]{FIGS/J0226corner_plot.png}
  %\includegraphics[scale = 0.21]{hexbinTurb/TURBcomp1_hexbin_chisq_1_J0226.png}
 \caption{LPs-J0226}
 \label{fig:lines-2b}
\end{figure*}
\newpage








\begin{figure*}
\centering
 \includegraphics[scale = 0.25]{spectra/J0305-A-_allspec.png}
 \includegraphics[scale = 0.25]{spectra/J0305-B-_allspec.png}
   \includegraphics[scale = 0.23]{bestfit/J0305_line_dust_bestsolnsTURB.png}
  \includegraphics[scale = 0.23]{bestfit/J0305_line_dust_bestsolns2COMP.png}
 \caption{LPs-J0305}
 \label{fig:lines-3a}
\end{figure*}

\newpage


\begin{figure*}
\centering
  \includegraphics[scale = 0.38]{FIGS/J0305corner_plot.png}
 \caption{LPs-J0305}
 \label{fig:lines-3b}
\end{figure*}
\newpage





\begin{figure*}
\centering
 \includegraphics[scale = 0.25]{spectra/J0748-A-_allspec.png}
 \includegraphics[scale = 0.25]{spectra/J0748-B-_allspec.png}
\includegraphics[scale = 0.23]{bestfit/J0748_line_dust_bestsolnsTURB.png}
  \includegraphics[scale = 0.23]{bestfit/J0748_line_dust_bestsolns2COMP.png}
 \caption{LPs-J0748}
 \label{fig:lines-4a}
\end{figure*}
\newpage

\begin{figure*}
\centering
  \includegraphics[scale = 0.38]{FIGS/J0748corner_plot.png}
 \caption{LPs-J0748}
 \label{fig:lines-4b}
\end{figure*}
\newpage



\begin{figure*}
\centering
 \includegraphics[scale = 0.25]{spectra/J0846-A-_allspec.png}
 \includegraphics[scale = 0.25]{spectra/J0846-B-_allspec.png}
 \includegraphics[scale = 0.23]{bestfit/J0846_line_dust_bestsolnsTURB.png}
  \includegraphics[scale = 0.23]{bestfit/J0846_line_dust_bestsolns2COMP.png}
 \caption{LPs-J0846}
 \label{fig:lines-5a}
\end{figure*}

\newpage



\begin{figure*}
\centering
  \includegraphics[scale = 0.38]{FIGS/J0846corner_plot.png}
 \caption{LPs-J0846}
 \label{fig:lines-5b}
\end{figure*}
\newpage








\begin{figure*}
\centering
 \includegraphics[scale = 0.25]{spectra/J105322-A-_allspec.png}
 \includegraphics[scale = 0.25]{spectra/J105322-B-_allspec.png}
  \includegraphics[scale = 0.23]{bestfit/J105322_line_dust_bestsolnsTURB.png}
  \includegraphics[scale = 0.23]{bestfit/J105322_line_dust_bestsolns2COMP.png}
 \caption{LPs-J105322}
 \label{fig:lines-6a}
\end{figure*}

\newpage




\begin{figure*}
\centering
  \includegraphics[scale = 0.38]{FIGS/J105322corner_plot.png}
 \caption{LPs-J105322}
 \label{fig:lines-6b}
\end{figure*}
\newpage




\begin{figure*}
\centering
 \includegraphics[scale = 0.25]{spectra/J105353-A-_allspec.png}
 \includegraphics[scale = 0.25]{spectra/J105353-B-_allspec.png}
 \includegraphics[scale = 0.25]{spectra/J105353-C-_allspec.png}
 \caption{LPs-J105353}
 \label{fig:lines-7a}
\end{figure*}


\begin{figure*}
\centering
   \includegraphics[scale = 0.23]{bestfit/J105353_line_dust_bestsolnsTURB.png}
  \includegraphics[scale = 0.23]{bestfit/J105353_line_dust_bestsolns2COMP.png}
 \caption{LPs-J105353}
 \label{fig:lines-7b}
\end{figure*}


\newpage


\begin{figure*}
\centering
  \includegraphics[scale = 0.38]{FIGS/J105353corner_plot.png}
 \caption{LPs-J105353}
 \label{fig:lines-7c}
\end{figure*}
\newpage



\begin{figure*}
\centering
 \includegraphics[scale = 0.25]{spectra/J112713_allspec.png}
    \includegraphics[scale = 0.23]{bestfit/J112713_line_dust_bestsolnsTURB.png}
  \includegraphics[scale = 0.23]{bestfit/J112713_line_dust_bestsolns2COMP.png}
 \caption{LPs-J112713}
 \label{fig:lines-8a}
\end{figure*}
\newpage





\begin{figure*}
\centering
  \includegraphics[scale = 0.38]{FIGS/J112713corner_plot.png}
 \caption{LPs-J112713}
 \label{fig:lines-8b}
\end{figure*}
\newpage



\begin{figure*}
\centering
 \includegraphics[scale = 0.25]{spectra/J112714-A-_allspec.png}
 \includegraphics[scale = 0.25]{spectra/J112714-B-_allspec.png}
     \includegraphics[scale = 0.23]{bestfit/J112714_line_dust_bestsolnsTURB.png}
  \includegraphics[scale = 0.23]{bestfit/J112714_line_dust_bestsolns2COMP.png}
 \caption{LPs-J112714}
 \label{fig:lines-9a}
\end{figure*}
\newpage


\begin{figure*}
\centering
  \includegraphics[scale = 0.38]{FIGS/J112714corner_plot.png}
 \caption{LPs-J112714}
 \label{fig:lines-9b}
\end{figure*}
\newpage







\begin{figure*}
\centering
 \includegraphics[scale = 0.25]{spectra/J1138-A-_allspec.png}
 \includegraphics[scale = 0.25]{spectra/J1138-B-_allspec.png}
      \includegraphics[scale = 0.23]{bestfit/J1138_line_dust_bestsolnsTURB.png}
  \includegraphics[scale = 0.23]{bestfit/J1138_line_dust_bestsolns2COMP.png}
 \caption{LPs-J1138}
 \label{fig:lines-10a}
\end{figure*}

\newpage




\begin{figure*}
\centering
  \includegraphics[scale = 0.38]{FIGS/J1138corner_plot.png}
 \caption{LPs-J1138}
 \label{fig:lines-10b}
\end{figure*}
\newpage


\begin{figure*}
\centering
 \includegraphics[scale = 0.25]{spectra/J1139-A-_allspec.png}
 \includegraphics[scale = 0.25]{spectra/J1139-B-_allspec.png}
 \includegraphics[scale = 0.23]{bestfit/J1139_line_dust_bestsolnsTURB.png}
  \includegraphics[scale = 0.23]{bestfit/J1139_line_dust_bestsolns2COMP.png}
 \caption{LPs-J1139}
 \label{fig:lines-11a}
\end{figure*}

\newpage

\begin{figure*}
\centering
  \includegraphics[scale = 0.38]{FIGS/J1139corner_plot.png}
 \caption{LPs-J1139}
 \label{fig:lines-11b}
\end{figure*}
\newpage





\begin{figure*}
\centering
 \includegraphics[scale = 0.25]{spectra/J1202-A-_allspec.png}
 \includegraphics[scale = 0.25]{spectra/J1202-B-_allspec.png}
 \includegraphics[scale = 0.25]{spectra/J1202-C-_allspec.png}
 \includegraphics[scale = 0.23]{bestfit/J1202_line_dust_bestsolnsTURB.png}
  \includegraphics[scale = 0.23]{bestfit/J1202_line_dust_bestsolns2COMP.png}
  \caption{LPs-J1202}
 \label{fig:lines-12a}
\end{figure*}


\newpage




\begin{figure*}
\centering
  \includegraphics[scale = 0.38]{FIGS/J1202corner_plot.png}
 \caption{LPs-J1202}
 \label{fig:lines-12b}
\end{figure*}
\newpage








\begin{figure*}
\centering
 \includegraphics[scale = 0.25]{spectra/J1322-A-_allspec.png}
 \includegraphics[scale = 0.25]{spectra/J1322-B-_allspec.png}
 \includegraphics[scale = 0.25]{spectra/J1322-C-_allspec.png}
  \includegraphics[scale = 0.23]{bestfit/J1322_line_dust_bestsolnsTURB.png}
  \includegraphics[scale = 0.23]{bestfit/J1322_line_dust_bestsolns2COMP.png}
 \caption{LPs-J1322}
 \label{fig:lines-13a}
\end{figure*}

\newpage



\begin{figure*}
\centering
  \includegraphics[scale = 0.38]{FIGS/J1322corner_plot.png}
 \caption{LPs-J1322}
 \label{fig:lines-13b}
\end{figure*}
\newpage











\begin{figure*}
\centering
 \includegraphics[scale = 0.25]{spectra/J1323-A-_allspec.png}
 \includegraphics[scale = 0.25]{spectra/J1323-B-_allspec.png}
 \includegraphics[scale = 0.25]{spectra/J1323-C-_allspec.png}
   \includegraphics[scale = 0.23]{bestfit/J1323_line_dust_bestsolnsTURB.png}
  \includegraphics[scale = 0.23]{bestfit/J1323_line_dust_bestsolns2COMP.png}
 \caption{LPs-J1323}
 \label{fig:lines-14a}
\end{figure*}
\newpage



\begin{figure*}
\centering
  \includegraphics[scale = 0.38]{FIGS/J1323corner_plot.png}
 \caption{LPs-J1323}
 \label{fig:lines-14b}
\end{figure*}
\newpage







\begin{figure*}
\centering
 \includegraphics[scale = 0.25]{spectra/J1326-A-_allspec.png}
 \includegraphics[scale = 0.25]{spectra/J1326-B-_allspec.png}
 \includegraphics[scale = 0.25]{spectra/J1326-C-_allspec.png}
   \includegraphics[scale = 0.23]{bestfit/J1326_line_dust_bestsolnsTURB.png}
  \includegraphics[scale = 0.23]{bestfit/J1326_line_dust_bestsolns2COMP.png}
 \caption{LPs-J1326}
 \label{fig:lines-15a}
\end{figure*}

\newpage



\begin{figure*}
\centering
  \includegraphics[scale = 0.38]{FIGS/J1326corner_plot.png}
 \caption{LPs-J1326}
 \label{fig:lines-15b}
\end{figure*}
\newpage




\begin{figure*}
\centering
 \includegraphics[scale = 0.25]{spectra/J1329-A-_allspec.png}
 \includegraphics[scale = 0.25]{spectra/J1329-B-_allspec.png}
 \includegraphics[scale = 0.25]{spectra/J1329-C-_allspec.png}
    \includegraphics[scale = 0.23]{bestfit/J1329_line_dust_bestsolnsTURB.png}
  \includegraphics[scale = 0.23]{bestfit/J1329_line_dust_bestsolns2COMP.png}
 \caption{LPs-J1329}
 \label{fig:lines-16a}
\end{figure*}
\newpage



\begin{figure*}
\centering
  \includegraphics[scale = 0.38]{FIGS/J1329corner_plot.png}
 \caption{LPs-J1329}
 \label{fig:lines-16b}
\end{figure*}
\newpage













\begin{figure*}
\centering
 \includegraphics[scale = 0.25]{spectra/J1336-A-_allspec.png}
 \includegraphics[scale = 0.25]{spectra/J1336-B-_allspec.png}
 \includegraphics[scale = 0.25]{spectra/J1336-C-_allspec.png}
 \caption{LPs-J1336}
 \label{fig:lines-17a}
\end{figure*}


\begin{figure*}
\centering
    \includegraphics[scale = 0.23]{bestfit/J1336_line_dust_bestsolnsTURB.png}
  \includegraphics[scale = 0.23]{bestfit/J1336_line_dust_bestsolns2COMP.png}
 \caption{LPs-J1336}
 \label{fig:lines-17b}
\end{figure*}

\newpage


\begin{figure*}
\centering
  \includegraphics[scale = 0.38]{FIGS/J1336corner_plot.png}
 \caption{LPs-J1336}
 \label{fig:lines-17c}
\end{figure*}
\newpage






\begin{figure*}
\centering
 \includegraphics[scale = 0.25]{spectra/J1428-A-_allspec.png}
 \includegraphics[scale = 0.25]{spectra/J1428-B-_allspec.png}
     \includegraphics[scale = 0.23]{bestfit/J1428_line_dust_bestsolnsTURB.png}
  \includegraphics[scale = 0.23]{bestfit/J1428_line_dust_bestsolns2COMP.png}
 \caption{LPs-J1428}
 \label{fig:lines-18a}
\end{figure*}

\newpage



\begin{figure*}
\centering
  \includegraphics[scale = 0.38]{FIGS/J1428corner_plot.png}
 \caption{LPs-J1428}
 \label{fig:lines-18b}
\end{figure*}
\newpage





\begin{figure*}
\centering
 \includegraphics[scale = 0.25]{spectra/J1449-A-_allspec.png}
 \includegraphics[scale = 0.25]{spectra/J1449-B-_allspec.png}
 \includegraphics[scale = 0.23]{bestfit/J1449_line_dust_bestsolnsTURB.png}
  \includegraphics[scale = 0.23]{bestfit/J1449_line_dust_bestsolns2COMP.png}
 \caption{LPs-J1449}
 \label{fig:lines-19a}
\end{figure*}
\newpage



\begin{figure*}
\centering
\includegraphics[scale = 0.38]{FIGS/J1449corner_plot.png}
 \caption{LPs-J1449}
 \label{fig:lines-19b}
\end{figure*}
\newpage




\begin{figure*}
\centering
 \includegraphics[scale = 0.25]{spectra/J1544_allspec.png}
 \includegraphics[scale = 0.23]{bestfit/J1544_line_dust_bestsolnsTURB.png}
  \includegraphics[scale = 0.23]{bestfit/J1544_line_dust_bestsolns2COMP.png}
 \caption{LPs-J1544}
 \label{fig:lines-20a}
\end{figure*}

\newpage

\begin{figure*}
\centering
  \includegraphics[scale = 0.38]{FIGS/J1544corner_plot.png}
 \caption{LPs-J1544}
 \label{fig:lines-20b}
\end{figure*}
\newpage










\begin{figure*}
\centering
 \includegraphics[scale = 0.25]{spectra/J1607-A-_allspec.png}
 \includegraphics[scale = 0.25]{spectra/J1607-B-_allspec.png}
  \includegraphics[scale = 0.23]{bestfit/J1607_line_dust_bestsolnsTURB.png}
  \includegraphics[scale = 0.23]{bestfit/J1607_line_dust_bestsolns2COMP.png}
 \caption{LPs-J1607}
 \label{fig:lines-21a}
\end{figure*}
\newpage


\begin{figure*}
\centering
  \includegraphics[scale = 0.38]{FIGS/J1607corner_plot.png}
 \caption{LPs-J1607}
 \label{fig:lines-21b}
\end{figure*}

\newpage






\begin{figure*}
\centering
 \includegraphics[scale = 0.25]{spectra/J1609-A-_allspec.png}
 \includegraphics[scale = 0.25]{spectra/J1609-B-_allspec.png}
  \includegraphics[scale = 0.25]{spectra/J1609-C-_allspec.png}
 \caption{LPs-J1609}
 \label{fig:lines-22}
\end{figure*}



\begin{figure*}
\centering
    \includegraphics[scale = 0.23]{bestfit/J1609_line_dust_bestsolnsTURB.png}
  \includegraphics[scale = 0.23]{bestfit/J1609_line_dust_bestsolns2COMP.png}
 \caption{LPs-J1609}
 \label{fig:lines-22}
\end{figure*}

\newpage


\begin{figure*}
\centering
  \includegraphics[scale = 0.38]{FIGS/J1609corner_plot.png}
 \caption{LPs-J1609}
 \label{fig:lines-22c}
\end{figure*}
\newpage









\begin{figure*}
\centering
 \includegraphics[scale = 0.25]{spectra/J2313-A-_allspec.png}
 \includegraphics[scale = 0.25]{spectra/J2313-B-_allspec.png}
     \includegraphics[scale = 0.23]{bestfit/J2313_line_dust_bestsolnsTURB.png}
  \includegraphics[scale = 0.23]{bestfit/J2313_line_dust_bestsolns2COMP.png}
 \caption{LPs-J2313}
 \label{fig:lines-23a}
\end{figure*}
\newpage



\begin{figure*}
\centering
    \includegraphics[scale = 0.38]{FIGS/J2313corner_plot.png}
 \caption{LPs-J2313}
 \label{fig:lines-23b}
\end{figure*}




